Prompt Consistency for Zero-Shot Task Generalization

One of the most impressive results of recent NLP history is the ability of pre-trained language models to solve new tasks in a zero-shot setting. To achieve this, NLP tasks are framed as natural language prompts, generating a response indicating the predicted output. Nonetheless, the performance in such settings often lags far behind its supervised counterpart, suggesting a large space for potential improvement. In this paper, we explore methods to utilize unlabeled data to improve zero-shot performance. Specifically, we take advantage of the fact that multiple prompts can be used to specify a single task, and propose to regularize prompt consistency, encouraging consistent predictions over this diverse set of prompts. Our method makes it possible to fine-tune the model either with extra unlabeled training data, or directly on test input at inference time in an unsupervised manner. In experiments, our approach outperforms the state-of-the-art zero-shot learner, T0 (Sanh et al., 2022), on 9 out of 11 datasets across 4 NLP tasks by up to 10.6 absolute points in terms of accuracy. The gains are often attained with a small number of unlabeled examples.

==> related_work.tex <==
\section{Background and Related Work}
\subsection{Multitask Prompted Training for Zero-shot Task Generalization}
\subsection{Unsupervised learning} data augmentation, ours is different in that we don't need large amount of unlabeled data, our model can be applied anytime we have a data set to test on, we make the model robust across prompts. Our model also provides a way to continual learning pre-trained models.
\subsection{Ensemble of multiple prompts} they are supervised learning
